Robust Self-Supervised LiDAR Odometry via Representative Structure Discovery and 3D Inherent Error Modeling

The correct ego-motion estimation basically relies on the understanding of correspondences between adjacent LiDAR scans. However, given the complex scenarios and the low-resolution LiDAR, finding reliable structures for identifying correspondences can be challenging. In this paper, we delve into structure reliability for accurate self-supervised ego-motion estimation and aim to alleviate the influence of unreliable structures in training, inference and mapping phases. We improve the self-supervised LiDAR odometry substantially from three aspects: 1) A two-stage odometry estimation network is developed, where we obtain the ego-motion by estimating a set of sub-region transformations and averaging them with a motion voting mechanism, to encourage the network focusing on representative structures. 2) The inherent alignment errors, which cannot be eliminated via ego-motion optimization, are down-weighted in losses based on the 3D point covariance estimations. 3) The discovered representative structures and learned point covariances are incorporated in the mapping module to improve the robustness of map construction. Our two-frame odometry outperforms the previous state of the arts by 16%/12% in terms of translational/rotational errors on the KITTI dataset and performs consistently well on the Apollo-Southbay datasets. We can even rival the fully supervised counterparts with our mapping module and more unlabeled training data.

==> doc/related.tex <==

% \input{fig/mapping.tex}
\vspace{-0.3ex}
\textbf{Classic LiDAR Odometry.}
% LiDAR odometry algorithms can be categorized as two-frame methods~\cite{arun1987least,segal2009generalized,serafin2015nicp} and multi-frame methods~\cite{zhang2014loam,shan2018lego}.
Classic approaches to LiDAR odometry are basically based on the point registration idea, where ICP~\cite{arun1987least}  and its variants~\cite{rusinkiewicz2001efficient,segal2009generalized,serafin2015nicp,pathak2010fast,velas2016collar} are commonly adopted.
% The classic two-frame methods are mostly based on the point registration, where ICP~\cite{arun1987least} and its variants~\cite{rusinkiewicz2001efficient,segal2009generalized,serafin2015nicp,pathak2010fast} are typical exemplars. 
The ICP algorithm identifies point correspondences and optimizes for the optimal pose transformation by minimizing the distances between the correspondence points iteratively.  These methods assume an ideal rigid transformation between LiDAR scans, which may fail to model the inherent errors caused by noise and moving objects. 
% The ICP iteratively finds the point correspondences and optimizes for the pose transformation between two LiDAR pointclouds util convergence. 
% Different ICP methods may apply different weights on the correspondence pairs during optimization 
% according to the geometric characteristics. 
% However they often fail to model the moving objects that 
% violate the algorithm assumption.
% Moreover, most of these methods are too computationally expensive to be applied in real-time systems. 
Due to the high computational cost,  
% of these algorithms,   
in practical odometry systems~\cite{zhang2014loam,shan2018lego,liosam2020shan}, ICP is generally conducted on some downsampled point clouds or manually selected sparse features~\cite{grant2013finding,steder2011point} to trade off the speed and accuracy. 
Besides, the LiDAR odometry systems usually include a mapping module~\cite{zhang2014loam,shan2018lego,liosam2020shan} running in the backend to overcome the sparsity of LiDAR scans by accumulating the scans as a more stable map which is used for pose refinement.  
% and correct the distortion of scanned point clouds 
% and further refine the pose estimation via scan-to-map alignment.  
These methods achieve low drift errors with the carefully designed hand-crafted features for map construction. %in the mapping refinement. 
Due to the absence of learning process, the features selected solely with the intuition and human understanding 
% of the scene, which 
may limit the 
% application 
generality to complicated scenarios.       

\textbf{Learning-based LiDAR Odometry.}
% Along with the rapid development of deep learning, 
With the development of deep learning, odometry estimation with deep neural networks have also been explored.  
% are being explored.  
The learning-based visual odometry was first investigated~\cite{konda2015learning,wang2017deepvo,zhou2017unsupervised, vijayanarasimhan2017sfm,li2019sequential,yang2020d3vo}.
These methods feed two or more consecutive color images to 2D neural networks to encode the visual appearance changing as high-dimensional features and predict the ego-motion based on these features.   
Following this line of thought, researchers~\cite{li2019net,velas2018cnn,chounsupervised} projected the LiDAR points onto a cylinder surface as 2D LiDAR images and then follow similar pipelines of learning-based visual odometry methods for LiDAR odometry.   
% adopt the similar pipeline of previous visual odometry methods for LiDAR odometry learning. 
However, during the cylindrical projection, some points on the same ray would be abandoned and the geometric information is thus inevitably lost.
% , since at each 2D image coordinate only one point can be retained if several points are projected to the same location.
Some recent works \cite{lu2019deepvcp,wang2019deep} proposed to formulate point registration problem with 3D neural networks \cite{qi2017pointnet,qi2017pointnet++}, which keep the 3D topology during feature encoding. However, these methods are still not efficient enough to be applied on large scale LiDAR data in real-time systems.  
%  may be projected to the same 2D location and only one point is finally retained. 
% The LiDAR can capture rich geometric information for ego-motion estimation
% and then borrowed the network architectures from the visual odometry methods. 
% Cho \etal~\cite{chounsupervised} extended this pipeline to unsupervised learning inspired by the unsupervised visual odometry~\cite{zhou2017unsupervised,li2018undeepvo}. 
More recently, 
% inspired by several 3D detection frameworks \cite{zhou2018voxelnet,yan2018second}, 
Xu \etal~\cite{xu2020selfvoxelo} propose a more efficient self-supervised LiDAR odometry framework based on 3D voxel representation which avoids the information losing caused by the cylindrical projection and enhances the 3D feature learning for odometry. However, they still have very limited network design for representative structure mining. 
% to handle the information losing problem caused by the cylindrical projection. 
% The previous learning-based LiDAR odometry requires the deep neural network to automatically recognize the reliable structures for ego-motion estimation and ignore the non-informative parts with no explicit mechanism applied to facilitate this process. 
% before predicting the ego-motion

% frameworks adopt a similar architecture  ask the network to understand the whole scene precisely 
% The conventional methods simply feed the LiDAR sweeps into an encoder network and expect the convolution layers to automatically extract the representative structures for ego-motion prediction. 


% further propose an efficient self-supervised LiDAR odometry network based on 3D voxel representation to handle the information losing problem caused by the cylindrical projection process.  

% naturally extract the 3D features from raw LiDAR points. 
% {However, the cylindrical projection may lose the spatially geometric structures of the input pointclouds, which leads to unreliable feature extraction. 

% \textbf{Feature Selection in Odometry}

==> fig/apollo_traj.tex <==
\begin{figure*}[tb!]
    \centering
    % \captionsetup[subfigure]{indention=10pt,font=small,margin=0pt,skip=0pt,position=top,labelformat=empty,} %labelformat=empty,
    % \resizebox{\linewidth}{!}{
        \begin{subfigure}[b]{0.99\linewidth} 
            \includegraphics[width=1\linewidth,trim={0cm 0cm 12cm 0cm},clip]{fig/traj_apollo.pdf}
        \end{subfigure} 
        \caption{
            Trajectory plots of different methods on Apollo-SouthBay dataset.
        }
    \vspace{-2ex}
	\label{fig:traj_apollo}
\end{figure*}

==> fig/arch.tex <==
\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.9\linewidth, trim=0cm 8cm 5cm 0cm, clip]{fig/framework.pdf}
    \includegraphics[angle=-90,origin=c, width=0.95\linewidth, trim=0cm 0cm 25cm 0cm, clip, ]{fig/arch.pdf}
    \caption{ The architecture of key modules in our proposed framework.  
    }
    \label{fig:arch}
    % \vspace{-3ex}
\end{figure}

==> fig/conf_vis.tex <==
\begin{figure*}[tb!]
    \centering
    \captionsetup[subfigure]{indention=10pt,font=small,margin=0pt,skip=0pt,position=top,labelformat=empty,} %labelformat=empty,
    % \resizebox{\linewidth}{!}{
        \begin{subfigure}[b]{0.45\linewidth} 
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_113.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_112.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_120.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_121.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_115.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_116.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_119.png}
            \caption{$\{w_{rot}^i\}$}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_118.png}
            \caption{$\{w_{tr}^i\}$}
        \end{subfigure} 
        % \begin{subfigure}[b]{0.45\linewidth} 
        %     % \caption{RGB Input}
        %     \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_099.png}
        % \end{subfigure} 
      
        % }
        
        \caption{
            The visualization of the 
            % top-performer selection 
            ego-motion voting  
            weights on KITTI and Apollo. The first column is the weights $\{w_{rot}^i\}$ for rotation predictions  and the second column is the weights $\{w_{tr}^i\}$ for translation predictions. The distant structures tends to be more valuable in rotation prediction while the distinctive structures, \eg corners, poles \etc, has more reliable translation predictions.  
            % We rescale the weights to logarithmic scale here for better visualization (the brighter the higher weight). 
            The brighter the higher weight.  
            Zoom in for better vision.
        }
        
    \vspace{-2ex}
	\label{fig:conf_vis}
\end{figure*}

==> fig/conf_vis_copy.tex <==
\begin{figure*}[b!]
    \centering
    \captionsetup[subfigure]{indention=10pt,font=small,margin=0pt,skip=0pt,position=top,labelformat=empty,} %labelformat=empty,
    % \resizebox{\linewidth}{!}{
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_089.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_090.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_091.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_092.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_101.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_094.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_095.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0.1cm 0cm 0cm 0.2cm},clip]{fig/vis/Selection_097.png}
        \end{subfigure} 
        % \begin{subfigure}[b]{0.45\linewidth} 
        %     % \caption{RGB Input}
        %     \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_099.png}
        % \end{subfigure} 
      
        % }
        
        \caption{
            The visualization of the top-performer selection weights on KITTI and Apollo.  We take the log scale here for better visualization (the brighter the higher weight). Zoom in for better vision.
        }
        
    \vspace{-2ex}
	\label{fig:conf_vis}
\end{figure*}

==> fig/cov_vis.tex <==
\begin{figure*}[tb!]
    \centering
    \captionsetup[subfigure]{indention=10pt,font=small,margin=0pt,skip=0pt,position=top,labelformat=empty,} %labelformat=empty,
    % \resizebox{\linewidth}{!}{
        \begin{subfigure}[b]{0.45\linewidth} 
            \includegraphics[width=1\linewidth,trim={0cm 5cm 0cm 3cm},clip]{fig/vis/Selection_107.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 5cm 0cm 3cm},clip]{fig/vis/Selection_109.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            \includegraphics[width=1\linewidth,trim={0cm 8cm 0cm 0cm},clip]{fig/vis/Selection_110.png}
        \end{subfigure} 
        \begin{subfigure}[b]{0.45\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 8cm 0cm 0cm},clip]{fig/vis/Selection_111.png}
        \end{subfigure} 
      
        % \begin{subfigure}[b]{0.45\linewidth} 
        %     % \caption{RGB Input}
        %     \includegraphics[width=1\linewidth,trim={0cm 0cm 0cm 0cm},clip]{fig/vis/Selection_099.png}
        % \end{subfigure} 
      
        % }
        \caption{
            By decomposing the covariance matrix estimations, we visualize the minimal eigenvalues' reciprocal (left column) and their corresponding eigenvectors (right column). For the visualization of eigenvalue reciprocals, the brighter the larger the value is. The nearby planar regions tends to have a lower variance in the normal directions while the remote areas and bushes with extreme sparse and noisy points tend to have higher uncertainties.
        }
        
    \vspace{-2ex}
	\label{fig:cov_vis}
\end{figure*}

==> fig/cov_vis_new.tex <==
\begin{figure}[tb!]
    \centering
    \captionsetup[subfigure]{indention=10pt,font=small,margin=0pt,skip=0pt,position=top,labelformat=empty,} %labelformat=empty,
    % \resizebox{\linewidth}{!}{
        \begin{subfigure}[b]{0.9\linewidth} 
            \includegraphics[width=1\linewidth,trim={0cm 5cm 0cm 9cm},clip]{fig/vis/Selection_107.png}
        \end{subfigure} 

        \begin{subfigure}[b]{0.9\linewidth} 
            % \caption{RGB Input}
            \includegraphics[width=1\linewidth,trim={0cm 5cm 0cm 9cm},clip]{fig/vis/Selection_109.png}
        \end{subfigure} 
        % \begin{subfigure}[b]{0.45\linewidth} 
        %     \includegraphics[width=1\linewidth,trim={0cm 8cm 0cm 0cm},clip]{fig/vis/Selection_110.png}
        % \end{subfigure} 
        % \begin{subfigure}[b]{0.45\linewidth} 
        %     % \caption{RGB Input}
        %     \includegraphics[width=1\linewidth,trim={0cm 8cm 0cm 0cm},clip]{fig/vis/Selection_111.png}
        % \end{subfigure} 
        % }
        \caption{
            By decomposing the covariance matrix estimations, we visualize the minimal eigenvalues' reciprocal (above) and their corresponding eigenvectors (below). For the eigenvalue reciprocals, the brighter the larger the value is.
            %  The nearby planar regions tends to have a lower variance in the normal directions while the remote areas and bushes with extreme sparse and noisy points tend to have higher uncertainties.
        }
        
    \vspace{-2ex}
	\label{fig:cov_vis}
\end{figure}

==> fig/fail.tex <==
\begin{figure}[b]
    \centering
    % \includegraphics[width=0.9\linewidth, trim=0cm 8cm 5cm 0cm, clip]{fig/framework.pdf}
    \includegraphics[width=0.9\linewidth, trim=0cm 11cm 23cm 0cm, clip]{fig/fail.pdf}
    \caption{
      Failure cases of our method.
      %  in the 2D birdview map and the 3D space. 
    }
    \label{fig:fail}
    \vspace{-3ex}
\end{figure}

==> fig/mapping.tex <==
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.95\linewidth, trim=0.5cm 11cm 33cm 1cm, clip]{fig/mapping.pdf}
    \caption{
      The diagram of our self-supervised odometry system. Given two consecutive LiDAR scans $S_{t-1}$ and $S_{t}$, our self-supervised 
      % ego-motion estimation network 
      two-frame odometry network discovers the representative structures $K_t$ and  
      estimates the ego-motion $\mathbf{T}^{pred}$. Meanwhile, the point covariances $C_t$ are also estimated for training robustness.  
      % uncertainty-aware training.  
      Then, all these estimations are sent to the mapping module for uncertainty-aware map construction and ego-motion refinement in the backend.   
    %  and point covariances $C_t$ for the latest scan. Then, all these estimations along with the representative structures $K_t$ discovered by the network are sent to the uncertainty-aware mapping module for map construction and ego-motion refinement in the backend.   
    }
    \label{fig:block_diagram}
    \vspace{-3ex}
\end{figure}

==> fig/traj.tex <==
\begin{figure}[tb]
    \centering
    % \includegraphics[width=0.9\linewidth, trim=0cm 8cm 5cm 0cm, clip]{fig/framework.pdf}
    % \includegraphics[width=0.9\linewidth, trim=0.5cm 3cm 3cm 0cm, clip]{fig/traj.pdf}
    % \includegraphics[width=0.9\linewidth, trim=0.5cm 13cm 2cm 0cm, clip]{fig/traj.pdf}
    \includegraphics[width=0.9\linewidth, trim=0.5cm 12.5cm 34cm 1.5cm, clip]{fig/traj2.pdf}
    \vspace{-2ex}
    \caption{
      % The plots of estimated trajectories by different methods from 2D-birdview (first row) and 3D-view (second row).
      % The plots of estimated trajectories by different methods from 2D-birdview and 3D-view side by side.
      The 3D visualization of estimated trajectories by different methods on KITTI sequences 09-10.
      %  in the 2D birdview map and the 3D space. 
    }
    \label{fig:traj_plot}
    \vspace{-3ex}
\end{figure}

==> table/eval_kitti_large.tex <==
\begin{table*}[t] 
    \caption{Comparison with state-of-the-art methods on KITTI odometry dataset. 
    We compare with other competitive classic methods, supervised methods and unsupervised methods to fully evaluate our performance. 
    % The Seq.~01 on highway is in a very open space with few structures to infer the agent's motions, where most of the unsupervised method and classic methods fail.
    % Some results were obtained from \cite{li2019net,chounsupervised}
    % We also list the supervised methods and visual odometry methods here for reference. 
    }
    %\vspace{-0.2cm}
    \label{tab:eval_kitti}
    % \begin{center}
      \centering
      % \tiny
      \resizebox{0.75\linewidth}{!}{
      \begin{tabular}{r|c|cccccccccccc}
        \hline
        % &\multicolumn{10}{|c|}{Classic Method} & 
        % \multicolumn{4}{|c|}{Supervised Method} & 
        % \multicolumn{10}{|c}{Unsupervised Method} \\
        % \hline
        &\multirow{2}{*}{Seq.} 
        % & \multicolumn{2}{|c|}{Training Seq.}
        &\multicolumn{2}{c|}{7}&
        \multicolumn{2}{c|}{8}
        &\multicolumn{2}{c|}{9}
        &\multicolumn{2}{c|}{10} 
        % &\multicolumn{2}{c|}{Training Avg.} 
        &\multicolumn{2}{c}{Avg.} \\
        \cline{3-12}

        &&\multicolumn{1}{c}{$t_{rel}$}&$r_{rel}$ 
        % &$t_{rel}$&$r_{rel}$ 
        &$t_{rel}$&$r_{rel}$
        &$t_{rel}$&$r_{rel}$
        &$t_{rel}$&$r_{rel}$
        &$t_{rel}$&$r_{rel}$ \\
        \hline\hline
        \multirow{7}{*}{\rotatebox{90}{Classic} } &ICP-po2po 
        % &6.45&3.16
        &5.17 &3.35 & 10.04&4.93&6.93&2.89&8.91&4.47 &7.76&3.98\\
        &ICP-po2pl 
        % &3.76&1.79
        &1.55 &1.42 & 4.42&2.14&3.95&1.71&6.13&2.60&4.01&1.97 \\
       
        &{CLS~\cite{velas2016collar}} 
        % &2.30&0.93
        &1.04 &0.73 & 2.14&1.05&1.95&0.92&3.46&1.28&2.15&1.00 \\
        &{NDT-P2D~\cite{stoyanov2012fast}} 
        % &34.2&5.73
        &7.51&3.07&13.6&4.62&33.7&7.06&20.5&3.06&18.8&4.45\\
        &{GICP~\cite{segal2009generalized}} 
        % &1.87&0.76
        &0.64 &0.45 & 1.58&0.75&1.97&0.77&1.31&0.62&1.38&0.65\\
        % &{LOAM~(w/o mapping)} &3.90&1.53&2.98 &1.55 & 4.89&2.04&6.04&1.79&3.65&1.55&4.39&1.73 \\
        % &{LOAM~(w/ mapping)~\cite{zhang2014loam}} &1.12&0.50&0.69 &0.50 & 1.18&0.44&1.20&0.48&1.51&0.57&1.15&0.50 \\
        &{LOAM~\cite{zhang2014loam}} &0.69 &0.50 & 1.18&0.44&1.20&0.48&1.51&0.57&1.15&0.50 \\
        &{LeGO-LOAM~\cite{shan2018lego}} &1.20 &0.59 & 1.59&0.61&1.51&0.63&1.99&0.68&1.57&0.63 \\
        % &{Lego-LOAM~\cite{shan2018lego}} &&& & & &&&&& \\
        \hline
       
        \multirow{3}{*}{\rotatebox{90}{Sup.} }
        &{Velas~\etal\cite{velas2018cnn}}  
        % &2.90&-&1.77 &- 
        & 2.89& - &4.94& - &3.27&-&3.22&- \\
        &{LO-Net~(w/o mapping)~\cite{li2019net}}  
        % &1.05&0.66
        &1.70 &0.89 & 2.12&{0.77}&1.37&0.58&1.80&0.93&1.75&0.79 \\
        &{LO-Net~(w/ mapping)~\cite{li2019net}}  
        % &0.71&0.45
        &0.56 &0.45 & {1.08}&0.43&0.77&0.38&{0.92}&0.41&{0.83}&0.42 \\
        \hline
        \multirow{6}{*}{\rotatebox{90}{Unsup.} }
        &Zhou~\etal*~\cite{zhou2017unsupervised}  
        % &30.8&4.63
        &21.3 &6.65 & 21.9&2.91&18.8&3.21& 14.3&3.30&19.1&4.02 \\ 
        &UnDeepVO*~\cite{li2018undeepvo}  
        % &4.80&2.69
        &3.15 &2.48 & 4.08&1.79&7.01&3.61& 10.6&4.65&6.22&3.13 \\ 
        &{Cho~\etal~\cite{chounsupervised}}  
        % &3.68&0.87
        &-&- & -& - &4.87&1.95& 5.02&1.83&4.95&1.89 \\ 
        &{Xu~\etal~( w/o mapping)\cite{xu2020selfvoxelo}}   
        % &2.50&1.11
        &3.09&1.81&3.16 & 1.14 &3.01&1.14& 3.48&1.11&3.19&1.30 \\ 
        &{Xu~\etal~(more data, w/o mapping)\cite{xu2020selfvoxelo}} 
        % &2.31&1.06
        &2.51&1.15&2.65 & 1.00 &2.86&1.17& 3.22&1.26&2.81&1.15  \\ 
        &{Xu~\etal(more data, w/ mapping)~\cite{xu2020selfvoxelo}} 
        % &{0.70}&{0.37}
        &$\mathbf{0.34}$&$\mathbf{0.21}$&{1.18} & $\mathbf{0.35}$ &{0.83}&{0.34}& {1.22}&{0.40}&{0.89}&{0.32} \\ 
        \cline{2-12}
        &Ours (w/o mapping) 
        % &2.12&0.93
        &3.24&1.72&2.48 &1.10  &2.75&1.01& 3.08&1.23&2.89&1.23 \\ 
        &Ours~(more data, w/o mapping ) 
        % &2.44&1.03
        &2.37&1.15& 2.14& 0.92 &2.61&1.05& 2.33&0.94&2.36&1.02 \\ 
        &Ours~(more data, w/ mapping) 
        % &\textbf{}&\textbf{}
        % &0.56&{0.26}&\textbf{1.18} & {0.40} &\textbf{0.65}&\textbf{0.25}& \textbf{0.72}&\textbf{0.31}&\textbf{0.78}&\textbf{0.31} \\ 
        &0.56&{0.26}&\textbf{1.17} & {0.38} &\textbf{0.65}&\textbf{0.25}& \textbf{0.72}&\textbf{0.31}&\textbf{0.78}&\textbf{0.31} \\ 
        \hline 
        
      \end{tabular}
      }
  
      {
        \raggedright 
        % \centering
        \scriptsize
        % ~~~~Following other unsupervised methods~\cite{chounsupervised,xu2020selfvoxelo}, the results of `Training Seq.' exclude the seq. 01 where most of the unsupervised method and classic methods fail due to the limited reliable features on highway. \\
        ~~~~$t_{rel}$ and $r_{rel}$ denote the average translational RMSE (\%) and rotational RMSE ($^\circ$/100m) on length of 100m-800m~\cite{geiger2012we}, and * denotes visual odometry methods. \\
       ~~~~`more data' indicates the training sequences are  (00-06, 11-22), otherwise the training sequences are (00-06) for our methods. Some results in this table are from \cite{li2019net}.
      % ~~~~$t_{rel}$: Average translational RMSE (\%) on length of 100m-800m~\cite{geiger2012we}. \\
      % ~~~~$r_{rel}$: Average rotational RMSE ($^\circ$/100m) on length of 100m-800m~\cite{geiger2012we}. \\
      % ~~~~*: Visual odometry methods.
      \par}
      \vspace{-3ex}
    % \end{center}
    % \end{threeparttable}
  \end{table*}



  % \begin{table*}[t] 
  %   \caption{Comparison with state-of-the-art methods on KITTI odometry dataset. 
  %   We compare with other competitive classic methods, supervised methods and unsupervised methods to fully evaluate our performance. 
  %   % The Seq.~01 on highway is in a very open space with few structures to infer the agent's motions, where most of the unsupervised method and classic methods fail.
  %   % Some results were obtained from \cite{li2019net,chounsupervised}
  %   % We also list the supervised methods and visual odometry methods here for reference. 
  %   }
  %   %\vspace{-0.2cm}
  %   \label{tab:eval_kitti}
  %   % \begin{center}
  %     \centering
  %     % \tiny
  %     \resizebox{0.8\linewidth}{!}{
  %     \begin{tabular}{rc|c|ccccccccccc}
  %       \hline
  %       % &\multicolumn{10}{|c|}{Classic Method} & 
  %       % \multicolumn{4}{|c|}{Supervised Method} & 
  %       % \multicolumn{10}{|c}{Unsupervised Method} \\
  %       % \hline
  %       &&\multirow{2}{*}{Seq.} 
  %       % & \multicolumn{2}{|c|}{Training Seq.}
  %       &&\multicolumn{2}{c|}{7}&
  %       \multicolumn{2}{c|}{8}
  %       &\multicolumn{2}{c|}{9}
  %       &\multicolumn{2}{c|}{10} 
  %       % &\multicolumn{2}{c|}{Training Avg.} 
  %       &\multicolumn{2}{c}{Avg.} \\
  %       \cline{4-13}

  %       &&&\multicolumn{1}{c}{$t_{rel}$}&$r_{rel}$ 
  %       % &$t_{rel}$&$r_{rel}$ 
  %       &$t_{rel}$&$r_{rel}$
  %       &$t_{rel}$&$r_{rel}$
  %       &$t_{rel}$&$r_{rel}$
  %       &$t_{rel}$&$r_{rel}$ \\
  %       \hline\hline
  %       \multirow{14}{*}{\rotatebox{90}{Two-frame} }&\multirow{7}{*}{\rotatebox{90}{Classic}} &ICP-po2po 
  %       % &6.45&3.16
  %       &5.17 &3.35 & 10.04&4.93&6.93&2.89&8.91&4.47 &7.76&3.98\\
  %       &&ICP-po2pl 
  %       % &3.76&1.79
  %       &1.55 &1.42 & 4.42&2.14&3.95&1.71&6.13&2.60&4.01&1.97 \\
       
  %       &&{CLS~\cite{velas2016collar}} 
  %       % &2.30&0.93
  %       &1.04 &0.73 & 2.14&1.05&1.95&0.92&3.46&1.28&2.15&1.00 \\
  %       &&{NDT-P2D~\cite{stoyanov2012fast}} 
  %       % &34.2&5.73
  %       &7.51&3.07&13.6&4.62&33.7&7.06&20.5&3.06&18.8&4.45\\
  %       &&{GICP~\cite{segal2009generalized}} 
  %       % &1.87&0.76
  %       &0.64 &0.45 & 1.58&0.75&1.97&0.77&1.31&0.62&1.38&0.65\\
  %       % &{LOAM~(w/o mapping)} &3.90&1.53&2.98 &1.55 & 4.89&2.04&6.04&1.79&3.65&1.55&4.39&1.73 \\
  %       % &{LOAM~(w/ mapping)~\cite{zhang2014loam}} &1.12&0.50&0.69 &0.50 & 1.18&0.44&1.20&0.48&1.51&0.57&1.15&0.50 \\
  %       &&{LOAM~\cite{zhang2014loam}} 
  %       % &1.12&0.50
  %       &0.69 &0.50 & 1.18&0.44&1.20&0.48&1.51&0.57&1.15&0.50 \\
  %       % &{Lego-LOAM~\cite{shan2018lego}} &&& & & &&&&& \\
  %       % \hline
  %       \cline{2-14}
       
  %       &\multirow{3}{*}{\rotatebox{90}{Sup.} }
  %       &{Velas~\etal\cite{velas2018cnn}}  
  %       % &2.90&-&1.77 &- 
  %       & 2.89& - &4.94& - &3.27&-&3.22&- \\
  %       &&{LO-Net~(w/o mapping)~\cite{li2019net}}  
  %       % &1.05&0.66
  %       &1.70 &0.89 & 2.12&{0.77}&1.37&0.58&1.80&0.93&1.75&0.79 \\
  %       &&{LO-Net~(w/ mapping)~\cite{li2019net}}  
  %       % &0.71&0.45
  %       &0.56 &0.45 & {1.08}&0.43&0.77&0.38&{0.92}&0.41&{0.83}&0.42 \\
  %       % \hline
  %       \cline{2-14}
  %       &\multirow{6}{*}{\rotatebox{90}{Unsup.} }
  %       &Zhou~\etal*~\cite{zhou2017unsupervised}  
  %       % &30.8&4.63
  %       &21.3 &6.65 & 21.9&2.91&18.8&3.21& 14.3&3.30&19.1&4.02 \\ 
  %       &&UnDeepVO*~\cite{li2018undeepvo}  
  %       % &4.80&2.69
  %       &3.15 &2.48 & 4.08&1.79&7.01&3.61& 10.6&4.65&6.22&3.13 \\ 
  %       &&{Cho~\etal~\cite{chounsupervised}}  
  %       % &3.68&0.87
  %       &-&- & -& - &4.87&1.95& 5.02&1.83&4.95&1.89 \\ 
  %       &&{Xu~\etal~( w/o mapping)\cite{xu2020selfvoxelo}}   
  %       % &2.50&1.11
  %       &3.09&1.81&3.16 & 1.14 &3.01&1.14& 3.48&1.11&3.19&1.30 \\ 
  %       &&{Xu~\etal~(more data, w/o mapping)\cite{xu2020selfvoxelo}} 
  %       % &2.31&1.06
  %       &2.51&1.15&2.65 & 1.00 &2.86&1.17& 3.22&1.26&2.81&1.15  \\ 
  %       &&{Xu~\etal(more data, w/ mapping)~\cite{xu2020selfvoxelo}} 
  %       % &{0.70}&{0.37}
  %       &$\mathbf{0.34}$&$\mathbf{0.21}$&{1.18} & $\mathbf{0.35}$ &{0.83}&{0.34}& {1.22}&{0.40}&{0.89}&{0.32} \\ 
  %       \cline{2-14}
  %       &&Ours 
  %       % &2.12&0.93
  %       &3.24&1.72&2.48 &1.10  &2.75&1.01& 3.08&1.23&2.89&1.23 \\ 
  %       &&Ours~(more data) 
  %       % &2.44&1.03
  %       &2.37&1.15& 2.14& 0.92 &2.61&1.05& 2.33&0.94&2.36&1.02 \\ 
  %       &&Ours~(more data, w/ mapping) 
  %       % &\textbf{}&\textbf{}
  %       &0.56&{0.26}&\textbf{1.18} & {0.40} &\textbf{0.65}&\textbf{0.25}& \textbf{0.72}&\textbf{0.31}&\textbf{0.78}&\textbf{0.31} \\ 
  %       \hline 
        
  %     \end{tabular}
  %     }
  
  %     {
  %       \raggedright 
  %       % \centering
  %       \scriptsize
  %       % ~~~~Following other unsupervised methods~\cite{chounsupervised,xu2020selfvoxelo}, the results of `Training Seq.' exclude the seq. 01 where most of the unsupervised method and classic methods fail due to the limited reliable features on highway. \\
  %       ~~~~$t_{rel}, r_{rel}$: Average translational RMSE (\%) and rotational RMSE ($^\circ$/100m) on length of 100m-800m~\cite{geiger2012we}.  \\
  %      ~~~~*: Visual odometry methods.
  %     % ~~~~$t_{rel}$: Average translational RMSE (\%) on length of 100m-800m~\cite{geiger2012we}. \\
  %     % ~~~~$r_{rel}$: Average rotational RMSE ($^\circ$/100m) on length of 100m-800m~\cite{geiger2012we}. \\
  %     % ~~~~*: Visual odometry methods.
  %     \par}
  %     \vspace{-4ex}
  %   % \end{center}
  %   % \end{threeparttable}
  % \end{table*}


==> table/runtime_compare.tex <==
\begin{table}
  \centering 
  % \vskip\baselineskip
  % \begin{minipage}[]{\textwidth}
    \centering
    % \parbox{1\linewidth}{
      \centering
    \captionof{table}{The runtime comparison among different methods.}\label{tab:runtime_comparison}
    \resizebox{0.4\linewidth}{!}{
      \begin{tabular}{c|*{2}{c}}
        \hline
        Methods & Time (ms) \\
        \hline 
        ICP-po2po~\cite{arun1987least} & 261\\
        ICP-po2pl~\cite{chen1992object} & 1250\\
        GICP~\cite{segal2009generalized} & 1781\\
        NDT-P2D~\cite{stoyanov2012fast} & 1723\\
        CLS~\cite{velas2016collar}& 19843 \\
        % LOAM & \\
        % LO-Net~\cite{li2019net} &\\
        Xu \etal~\cite{xu2020selfvoxelo} &88.4 \\
        \hline
        Ours & 97.9 \\
        \hline
      \end{tabular}
    }
    % }
    % \end{minipage}
  \end{table}

% \begin{table}[t] 
%     % \caption{The average runtime (ms) on KITTI Seq. 07-10 of each submodule in Fig.\ref{fig:framework}. }%\vspace{-0.2cm}
%       % \resizebox{0.9\linewidth}{!}{
%       \centering
%       \parbox{.45\linewidth}{
%       \vspace{-2ex}
%       \centering
%       \caption{The average runtime (ms) on KITTI Seq. 07-10 of each submodule in Fig.\ref{fig:framework}. }
%     \label{tab:runtime}
%       % \resizebox{0.95\linewidth}{!}{
%       \begin{tabular}{c|*{2}{c}}
%         \hline
%         Module & Time (ms) \\
%         \hline
%         Voxelization & 0.7\\
%         Voxel Feature Extraction & 66.4\\
%          Odometry Regression & 27.1 \\
%          \hline
%          Total & 94.2\\
%         \hline
%       \end{tabular}
%       % }
%       }
%     \hspace{6ex}
%     \parbox{0.45\linewidth}{
%       \centering
%       \caption{The runtime comparison among different methods.}
%     \label{tab:runtime_comparison}
%       % \resizebox{0.7\linewidth}{!}{
%       \begin{tabular}{c|*{2}{c}}
%         \hline
%         Methods & Time (ms) \\
%         \hline 
%         ICP~\cite{arun1987least} & 261\\
%         GICP~\cite{segal2009generalized} & 1781\\
%         NDT-P2D~\cite{stoyanov2012fast} & 1723\\
%         CLS~\cite{velas2016collar}& 19843 \\
%         % LOAM & \\
%         Ours&94.2 \\
%         \hline
%       \end{tabular}
%       % }
%       }
    
%   \end{table}

